Cogsworth: Byzantine View Synchronization

Most methods for Byzantine fault tolerance (BFT) in the partial synchrony setting divide the local state of the nodes into views, and the transition from one view to the next dictates a leader change. In order to provide liveness, all honest nodes need to stay in the same view for a sufficiently long time. This requires \emph{view synchronization}, a requisite of BFT that we extract and formally define here. Existing approaches for Byzantine view synchronization incur quadratic communication (in $n$, the number of parties). A cascade of $O(n)$ view changes may thus result in $O(n^3)$ communication complexity. This paper presents a new Byzantine view synchronization algorithm named Cogsworth, that has optimistically linear communication complexity and constant latency. Faced with benign failures, Cogsworth has expected linear communication and constant latency. The result here serves as an important step towards reaching solutions that have overall quadratic communication, the known lower bound on Byzantine fault tolerant consensus. Cogsworth is particularly useful for a family of BFT protocols that already exhibit linear communication under various circumstances, but suffer quadratic overhead due to view synchronization.

==> algs/round_doubling_v2.tex <==

\newcommand{\currDuration}{\ensuremath{\textit{view\_duration}}\xspace}
\newcommand{\wishVar}{\ensuremath{\textit{wish}}\xspace}
\newcommand{\firstRoundDuration}{\ensuremath{\beta}\xspace}

\begin{algorithm}[h] \footnotesize
	\caption{View doubling synchronizer for node $\process{}$}
	\label{alg:roundDoubling}
	\SetAlgoNoEnd
	\DontPrintSemicolon
	\SetInd{0.4em}{0.4em}

	\KwInitialize(:) {
%		$\wishVar \gets 0$ \;
		$\curr \gets 0$ \label{alg:roundDoubling:currInitialize} \;
		$\currDuration \gets \firstRoundDuration $ \commentx{\firstRoundDuration is a predefined value for the duration of the first view} \label{alg:roundDoubnling:durationInitialize} \;
	}

	\BlankLine

	\KwOn({$\wishToAdvance$: } \label{alg:roundDoubling:timeout}) {
		$\currDuration \gets \firstRoundDuration$ \;
		$\curr \gets \curr + 1$ \;
		\proposeRound{\curr}
	}
	
	\KwAfter({\currDuration has passed since last changing its value:} \label{alg:roundDoubling:internalTimeout})
	{
		$\curr \gets \curr + 1$ \;
		$\currDuration \gets 2 \times \currDuration$ \;
%		\If{ $\wishVar \ge \curr$ \label{alg:roundDoubling:ifCond}} 
%		{
			\proposeRound{\curr} \;
%		}
	}


\end{algorithm}

